LanSER: Language-Model Supported Speech Emotion Recognition

Speech emotion recognition (SER) models typically rely on costly human-labeled data for training, making scaling methods to large speech datasets and nuanced emotion taxonomies difficult. We present LanSER, a method that enables the use of unlabeled data by inferring weak emotion labels via pre-trained large language models through weakly-supervised learning. For inferring weak labels constrained to a taxonomy, we use a textual entailment approach that selects an emotion label with the highest entailment score for a speech transcript extracted via automatic speech recognition. Our experimental results show that models pre-trained on large datasets with this weak supervision outperform other baseline models on standard SER datasets when fine-tuned, and show improved label efficiency. Despite being pre-trained on labels derived only from text, we show that the resulting representations appear to model the prosodic content of speech.

==> discussion.tex <==
% \section{Discussion and Future Work}
% While we investigated various aspects in designing a weak-supervision algorithm from LLMs, we notice that there exist several possibilities to improve this idea. For better quality of weak labels, one can add additional contexts to the input context of LLMs. In addition, it would be an interesting direction to generate weak label with an open-set taxonomy, in order to maximize the expressiveness of LLMs. Finally, while we experimented with simple ResNet-50 as the backbone networks, exploring modern networks would be beneficial, such as conformer-based models~\cite{cap}.

% - Adding context
% - Open-ended weak label space
% - SOTA SER models
% - Utilizing both weakly-labeled and public labeled data (semi-supervised learning)
